Enabling Approximate Joint Sampling in Diffusion LMs

In autoregressive language models, each token is sampled by conditioning on all the past tokens; the overall string has thus been sampled from the correct underlying joint distribution represented by the model. In contrast, masked diffusion language models generate text by unmasking tokens out of order and potentially in parallel. Generating an overall string sampled from the correct underlying joint distribution would (again) require exactly one token unmasking in every full-model forward pass. The more tokens unmasked in parallel, the further away the string is from the true joint; this can be seen in the resulting drop in accuracy (but, increase in speed). In this paper we devise a way to {\em approximately} sample multiple tokens from the joint distribution in a single full-model forward pass; we do so by developing a new lightweight single-layer ``sampler" on top of an existing large diffusion LM. One forward pass of the full model can now be followed by multiple forward passes of only this sampler layer, to yield multiple unmasked tokens. Our sampler is trained to mimic exact joint sampling from the (frozen) full model. We show the effectiveness of our approximate joint sampling for both pretrained-only (Dream-7B-Base, Llada-7B-Base) and instruction-tuned (Dream-7B-Instruct, Dream-7B-Coder) models on language modeling and math \& coding tasks. When four tokens are unmasked for each full-model denoising step, our sampling algorithm achieves a MAUVE score of 0.87 (vs marginal baseline of 0.31) with respect to the true joint distribution.

==> archived.tex <==

\begin{table}[h]
\centering
\begin{tabular}{lccc}
\toprule
 & \textbf{Joint Sampling} & \multicolumn{2}{c}{\textbf{Marginal Sampling}} \\
\cmidrule(lr){2-2}\cmidrule(lr){3-4}
\textbf{Temperature} & \multicolumn{1}{c}{64 steps} & 64 steps & 128 steps \\
\midrule
0.0 & 69.69 & 63.63 & 73.48 \\
1.0 & 47.72 & 37.12 & 62.87 \\
\bottomrule
\end{tabular}
\caption{GSM8K accuracy on generation of 128 tokens}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{lccccc}
\toprule
 & \textbf{Joint Sampling} & \textbf{only KL} & \textbf{no Base MSE} & \multicolumn{2}{c}{\textbf{Marginal Sampling}} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-6}
\textbf{Temperature} & \multicolumn{3}{c}{64 steps} & 64 steps & 128 steps \\
\midrule
0.0 & 69.69 & 67.42 & 71.21 & 63.63 & 73.48 \\
1.0 & 47.72 & 35.60 & 39.39 & 37.12 & 62.87 \\
\bottomrule
\end{tabular}
\caption{GSM8K accuracy on generation of 128 tokens}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{lccccc}
\toprule
 & \textbf{Joint Sampling} & \textbf{only KL} & \textbf{no Base MSE} & \multicolumn{2}{c}{\textbf{Marginal Sampling}} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-6}
\textbf{Temperature} & \multicolumn{3}{c}{128 steps} & 128 steps & 256 steps \\
\midrule
0.0 & 12/51 & 12/53 & 11/53 & 11/51 &  17/63\\
1.0 & 4/15 & 5/16 & 5/21 & 6/18 &  10/44\\
\bottomrule
\end{tabular}
\caption{HumanEval/MBPP accuracy on generation of 256 tokens}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{lccccc}
\toprule
 & \textbf{Joint Sampling} & \multicolumn{2}{c}{\textbf{Marginal Sampling}} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-6}
\textbf{Temperature} &  & Conf-based & 256 steps \\
\midrule
0.0 & 12/51 & 12/53 & 11/53 & 11/51 &  17/63\\
1.0 & 4/15 & 5/16 & 5/21 & 6/18 &  10/44\\
\bottomrule
\end{tabular}
\caption{NLL numbers for 128 tokens}
\end{table}



\begin{table}[h]
\centering
\begin{tabular}{cccccc}
\toprule
& & Spec=0 & Spec=1 & Spec=2 & Spec=3 \\
% \cmidrule(lr){2-2}\cmidrule(lr){3-4}
\midrule
\multirow{2}{*}{0.3} & Marginal & & & & \\
 & Joint & & & & \\
\multirow{2}{*}{0.4} & Marginal & & & & \\
 & Joint & & & & \\
\multirow{2}{*}{0.5} & Marginal & & & & \\
 & Joint & & & & \\
\bottomrule
\end{tabular}
\caption{\label{table:adaptive_speculation_len_table} In this table we report the speculation length for the experimental setup in Table~\ref{table:adaptive_nll_table}}
\end{table}




==> pretraining_experiments.tex <==
\subsection{Results on Random Masking models}\label{subsec:mdlm_experiments}

\paragraph{Pretraining/continual-pretraining results on Text8}
Sequences are of length 256 and are tokenized at character level. Results presented in Tab~\ref{tab:resultsontext8}


\paragraph{Frozen-base results on OpenWebText}


\begin{table}[t]
\centering
\begin{tabular}{lcccc}
\toprule
& Sampling & \textbf{K=1} & \textbf{K=2} & \textbf{K=4} \\
\midrule
Std. Training (9 layers) & Marginal & 5.45 & 5.64 & 6.08 \\
Std. Training (8 layers) & Marginal & 5.77 & 5.97 & 6.40 \\
\midrule
\multirow{2}{*}{Joint (8+1 layers)} & Marginal & 5.95 & 6.24 & 6.66 \\
 & Joint & 5.99 & 5.80 & 5.72 \\
\midrule
\multirow{2}{*}{Continual-Joint (8+1 layers)} & Marginal & 5.76 & 5.91 & 6.36 \\
 & Joint & 5.69 & 5.77 & 5.84 \\
\bottomrule
\end{tabular}
\caption{\label{tab:resultsontext8} In this table we compare the NLL scores for text8 dataset. Evaluation is done using an auto-regressive model trained on the same text8 dataset. Models are trained for 80K iterations. The continually-pretrained model is trained for 40K iterations with just the base model and the remaining 40 with ADJUST joint training
}
\end{table}


\begin{table}[t]
\centering
\begin{tabular}{lccccccc}
\toprule
& Sampling & \multicolumn{2}{c}{\textbf{NFE=256}} & \multicolumn{2}{c}{\textbf{NFE=128}} & \multicolumn{2}{c}{\textbf{NFE=64}} \\
& & NLL & Entropy & NLL & Entropy & NLL & Entropy \\
\midrule
\multirow{2}{*}{Continual-Joint w/ frozen base} & Marginal & 53.14 & 5.47 & 58.69 & 5.50 & 70.33 & 5.53 \\
& Joint & 53.14 & 5.47 & 59.28 & 5.49 & 66.82 & 5.51\\
\multirow{2}{*}{Continual-Joint} & Marginal & 59.43 & 5.47 & 63.45 & 5.49 & 72.82 & 5.54\\
 & Joint & - & - & 61.88 & 5.49 & 66.34 & 5.51\\
\bottomrule
\end{tabular}
\caption{\label{tab:resultsontext8} In this table we compare the NLL scores and entropy for OWT dataset. These models are trained for 100K iterations starting from the base MDLM model. 
}
\end{table}

